CollisionIK: A Per-Instant Pose Optimization Method for Generating Robot Motions with Environment Collision Avoidance

In this work, we present a per-instant pose optimization method that can generate configurations that achieve specified pose or motion objectives as best as possible over a sequence of solutions, while also simultaneously avoiding collisions with static or dynamic obstacles in the environment. We cast our method as a multi-objective, non-linear constrained optimization-based IK problem where each term in the objective function encodes a particular pose objective. We demonstrate how to effectively incorporate environment collision avoidance as a single term in this multi-objective, optimization-based IK structure, and provide solutions for how to spatially represent and organize external environments such that data can be efficiently passed to a real-time, performance-critical optimization loop. We demonstrate the effectiveness of our method by comparing it to various state-of-the-art methods in a testbed of simulation experiments and discuss the implications of our work based on our results.

==> 0a-abstract.tex <==
\begin{abstract}
In this work, we present a method for generating robot motions on-the-fly that avoid collisions with static or dynamic obstacles in an environment, while also simultaneously accommodating any other motion objectives, such as matching specified end-effector pose goals or synthesizing smooth motion.  Our method is framed as a per-update, generalized inverse kinematics (IK) solver that outputs a stream of joint configurations as fast as possible in real-time.  We cast this generalized IK method as a multi-objective, non-linear constrained optimization problem.  The objective function is a weighted sum, where each term in the sum encodes a particular motion objective.  We demonstrate how to effectively incorporate environment collision avoidance as a single term in this multi-objective, optimization-based IK structure, and provide initial solutions for how to spatially represent and organize external environments such that data can be efficiently passed to a real-time, performance critical optimization loop.  We demonstrate the effectiveness of our method by comparing it to various state-of-the-art methods in a large testbed of simulation experiments and discuss the implications of our work based on our results.
\end{abstract}

%  In the context of robot motion synthesis, this structure builds on the relaxed inverse kinematics (RelaxedIK) paradigm, where the solver decides how to \textit{relax} certain objectives in favor of other, more important, terms in the case of competing objectives.

% This per-update IK paradigm, where motions are iteratively constructed on-the-fly, nicely allows the robot to react and adapt its motion to complex or dynamic environments, all while still reflecting other specified motion objectives as best as possible.


==> 0b-abstract.tex <==
\begin{abstract}
In this work, we present an inverse kinematics (IK) method that generates robot motions that achieve any specified motion objectives as best as possible over a sequence of solutions, while also simultaneously avoiding collisions with static or dynamic obstacles in the environment.  We cast this generalized IK method as a multi-objective, non-linear constrained optimization problem where each term in the objective function encodes a particular motion objective.  We demonstrate how to effectively incorporate environment collision avoidance as a single term in this multi-objective, optimization-based IK structure, and provide initial solutions for how to spatially represent and organize external environments such that data can be efficiently passed to a real-time, performance critical optimization loop.  We demonstrate the effectiveness of our method by comparing it to various state-of-the-art methods in a testbed of simulation experiments and discuss the implications of our work based on our results.
\end{abstract}

%  In the context of robot motion synthesis, this structure builds on the relaxed inverse kinematics (RelaxedIK) paradigm, where the solver decides how to \textit{relax} certain objectives in favor of other, more important, terms in the case of competing objectives.

% This per-update IK paradigm, where motions are iteratively constructed on-the-fly, nicely allows the robot to react and adapt its motion to complex or dynamic environments, all while still reflecting other specified motion objectives as best as possible.


==> 1a-intro.tex <==
\section{Introduction}
\label{sec:intro}

Generating motions for robot manipulators that avoid collisions with obstacles in an environment has long been a fundamental problem in robotics.  Common solutions for addressing this problem, such as sampling-based motion planners \cite{lavalle2006planning, kavraki1994probabilistic, lavalle1998rapidly, karaman2011sampling}, traditionally only focus on achieving short, collision-free paths from a start point to a goal point in the robot's configuration space.  However, to perform tasks in a variety of complex or dynamic environments, robot manipulators must be able to quickly calculate motions on-the-fly that achieve many simultaneous, potentially competing, motion objectives in \textit{addition} to avoiding collisions with people or objects in the environment.  For instance, a robot hygienist holding a mirror to improve a dentist's visibility during a procedure would not only have to avoid collisions with the patient or other fixtures in the room, but it would also have to continuously update its end-effector pose to consistently reflect a sufficient view, move smoothly without any discontinuous jerks in the motion, avoid kinematic singularities, and prevent self-collisions. 


In this work, we present a method for generating robot motions on-the-fly that avoid collisions with obstacles in the environment, while also simultaneously accommodating any other motion objectives.  Examples of additional motion objectives include matching specified end-effector pose goals; avoiding self-collisions; or smoothing joint velocities, accelerations, and jerks.  Our method is framed as a per-update, generalized inverse kinematics (IK) solver that outputs a stream of robot joint configurations as fast as possible in real-time.  This per-update IK paradigm, where motions are iteratively constructed on-the-fly, effectively allows the robot to react and adapt its motion to complex or dynamic environments, all while still reflecting other specified motion objectives as best as possible.

\begin{figure}[t!]
	\includegraphics[width=\columnwidth]{figures/figures-01.png}
	\caption{}
	\label{fig:teaser}
	\vspace{-3pt}
\end{figure}

We cast our generalized IK method as a multi-objective, non-linear constrained optimization problem.  The objective function is a weighted sum, where each term in the sum encodes a particular motion objective.  The weights on the terms in the objective function set importances of the various terms, and allows the optimization solver to \textit{relax} certain objectives in favor of other, more important, terms in the case of competing objectives.  In the context of robot motion generation, this builds on the paradigm called \textit{relaxed} inverse kinematics (RelaxedIK) in prior work \cite{rakita2018rss}.  Throughout this work, we overview the structure of this overall optimization framework and highlight how this or similar frameworks extend well to the case of environment collision avoidance.  

Our current work offers \textit{two} technical contributions: (1) We demonstrate how to effectively incorporate environment collision avoidance as a single term in a multi-objective, optimization-based IK structure \S\ref{}; and (2) We provide initial solutions for how to spatially represent and organize external environments such that data can be efficiently passed to a real-time, performance critical optimization loop \S\ref{}.  We also provide open-source code that implements our proposed method, available here: \textit{link will appear here}.    

We assessed the efficacy of our method by running a testbed of simulation experiments in large iterations.  We compared our method to the MoveIt! library Cartesian path controller \cite{chitta2012moveit} and \textit{RelaxedIK} \cite{rakita2018rss} on a number of simulated robots and tasks.  We demonstrate that our method successfully avoids collisions with static or dynamic objects in the environment in real-time, and also consistently achieves additional motion objectives.  We discuss the benefits and drawbacks of our method compared to the comparison cases, and conclude with an overall discussion about the implications of our work based on our results \S\ref{}.         




==> 1b-intro.tex <==
\section{Introduction}

In this work, we present a generalized inverse kinematics (IK) method, called \textit{CollisionIK}, that generates robot motions that achieve any specified motion objectives as best as possible over a sequence of solutions, while also simultaneously avoiding collisions with static or dynamic obstacles in the environment.  Examples of motion objectives that our method could achieve include traditional IK goals, such as matching a sequence of specified end-effector poses, but can include any arbitrary non-linear terms, such as keeping distance from self-collisions, smoothing joint motion, or avoiding kinematic singularities.  Our IK method outputs a stream of robot joint configurations in a per-update fashion as fast as possible in real-time.  This per-update IK paradigm, where motions are iteratively constructed on-the-fly, effectively allows the robot to react and adapt its motion to complex or dynamic environments, all while still reflecting other specified objectives as best as possible.

We cast our generalized IK method as a multi-objective, non-linear constrained optimization problem.  The objective function is a weighted sum, where each term in the sum encodes a particular motion objective.  The weights on the terms in the objective function set importances of the various terms, and allows the optimization solver to \textit{relax} certain objectives in favor of other, more important, terms in the case of competing objectives.  In the context of robot motion generation, this builds on the paradigm called \textit{relaxed} inverse kinematics (RelaxedIK) in prior work \cite{rakita2018rss}.  Throughout this work, we overview the structure of this overall optimization framework and highlight how this or similar frameworks extend well to the case of environment collision avoidance. 

Our current work offers \textit{two} technical contributions: (1) We demonstrate how to effectively incorporate environment collision avoidance as a single term in a multi-objective, optimization-based IK structure (\S\ref{sec:objective_term}); and (2) We provide initial solutions for how to spatially represent and organize external environments such that data can be efficiently passed to a real-time, performance critical optimization loop (\S\ref{sec:env_representation} and \S\ref{sec:collision_scene_filtering}).   We also provide open-source code that implements our proposed method\footnote{[link will appear here]}.    

\begin{figure}[t!]
	\includegraphics[width=\columnwidth]{figures/figures-01.png}
	\caption{}
	\label{fig:teaser}
	\vspace{3pt}
\end{figure}

We assessed the efficacy of our method by running a testbed of simulation experiments (\S\ref{sec:evaluation}).  We compared our method to the MoveIt! library Cartesian path controller \cite{chitta2012moveit} and \textit{RelaxedIK} \cite{rakita2018rss} on various simulated robots and tasks.  We demonstrate that our method successfully avoids collisions with static or dynamic objects in the environment in real-time, and also consistently achieves additional motion objectives.  We also show that our method scales well and maintains its efficient performance even in environments with many obstacles.  We discuss the benefits and drawbacks of our method compared to the alternative approaches, and conclude with an overall discussion about the implications of our work based on our results (\S\ref{sec:discussion}).   




